TempCLR: Temporal Alignment Representation with Contrastive Learning

Video representation learning has been successful in video-text pre-training for zero-shot transfer, where each sentence is trained to be close to the paired video clips in a common feature space. For long videos, given a paragraph of description where the sentences describe different segments of the video, by matching all sentence-clip pairs, the paragraph and the full video are aligned implicitly. However, such unit-level comparison may ignore global temporal context, which inevitably limits the generalization ability. In this paper, we propose a contrastive learning framework TempCLR to compare the full video and the paragraph explicitly. As the video/paragraph is formulated as a sequence of clips/sentences, under the constraint of their temporal order, we use dynamic time warping to compute the minimum cumulative cost over sentence-clip pairs as the sequence-level distance. To explore the temporal dynamics, we break the consistency of temporal succession by shuffling video clips w.r.t. temporal granularity. Then, we obtain the representations for clips/sentences, which perceive the temporal information and thus facilitate the sequence alignment. In addition to pre-training on the video and paragraph, our approach can also generalize on the matching between video instances. We evaluate our approach on video retrieval, action step localization, and few-shot action recognition, and achieve consistent performance gain over all three tasks. Detailed ablation studies are provided to justify the approach design.

==> result/table_ablation1.tex <==
\begin{table}[]
    \parbox{.31\textwidth}
    {
        \centering
        \caption{Negative sampling}
        \resizebox{.31\textwidth}{!}
        {%
            \begin{tabular}{c|c}
                \hlineB{3}
                Negative Strategy & Recall \\
                \hline
                un-paired & 48.0\\
                all-unit & 49.3 \\
                within-seg & 46.4 \\
                seg-only & \underline{52.1} \\
                seg-unit & \textbf{52.5} \\
                visual-anchor & 52.0 \\
                \hlineB{3}
            \end{tabular}
        }\label{tab:negative}
    }
    \hfill
    \parbox{.68\textwidth}
    {
        \centering
        \caption{Performance comparison on action recognition}
        \resizebox{.68\textwidth}{!}
        {%
            \renewcommand{\arraystretch}{1.05}
            \begin{tabular}{l|cc}
                \hlineB{3}
                Approach & 1-shot & 5-shot \\
                \hline
                TSN++*   & 33.6 & 43   \\
                CMN++*   & 34.4 & 43.8 \\
                RTRN++*  & 38.6 & 48.9 \\
                OTAM~\citep{cao2020few}    & 42.8 & 52.3 \\
                RTX~\citep{perrett2021temporal}     & 42   & 64.6 \\
                MTFAN~\citep{wu2022motion}   & 45.4 & 60.4 \\
                \approach{} (Ours) & \textbf{47.8} & \textbf{66.5} \\
                \hlineB{3}
                \multicolumn{3}{l}{*:Results are reported in \citet{cao2020few}}
            \end{tabular}
        }\label{tab:fsar}
    }
\end{table}
